SmartInv: Multimodal Learning for Smart Contract Invariant Inference

Smart contracts are software programs that enable diverse business activities on the blockchain. Recent research has identified new classes of "machine un-auditable" bugs that arise from both transactional contexts and source code. Existing detection methods require human understanding of underlying transaction logic and manual reasoning across different sources of context (i.e. modalities), such as code, dynamic transaction executions, and natural language specifying the expected transaction behavior. To automate the detection of ``machine un-auditable'' bugs, we present SmartInv, an accurate and fast smart contract invariant inference framework. Our key insight is that the expected behavior of smart contracts, as specified by invariants, relies on understanding and reasoning across multimodal information, such as source code and natural language. We propose a new prompting strategy to foundation models, Tier of Thought (ToT), to reason across multiple modalities of smart contracts and ultimately to generate invariants. By checking the violation of these generated invariants, SmartInv can identify potential vulnerabilities. We evaluate SmartInv on real-world contracts and re-discover bugs that resulted in multi-million dollar losses over the past 2.5 years (from January 1, 2021 to May 31, 2023). Our extensive evaluation shows that SmartInv generates (3.5X) more bug-critical invariants and detects (4$\times$) more critical bugs compared to the state-of-the-art tools in significantly (150X) less time. \sys uncovers 119 zero-day vulnerabilities from the 89,621 real-world contracts. Among them, five are critical zero-day bugs confirmed by developers as ``high severity.''

==> abstract_0_.tex <==
\begin{abstract}

Smart contracts are software programs enabling blockchain users' diverse business activities. Recent research has identified new classes of ``machine un-auditable'' bugs stemming from both transactional contexts and source code. Detecting them often require manual reasoning based on expert understanding of the underlying transaction logic. A typical approach is to manually specify invariants based on human reasoning of transactional contexts and source code. Unfortunately, manual specification is labor intensive and unscalable. Existing automated tools have fundamental limitations. Specifically, they cannot reason across various source of information (\ie modalities), such as code, dynamic transaction executions, natural language. Hence, existing automated tools cannot detect the increasingly prevalent high-impact bugs. 

We present \sys, an accurate and fast smart contract invariant inference framework to detect bugs in pre-deployment smart contracts. Our key insight is that the expected behavior of smart contracts, as specified by invariants, relies on understanding and reasoning across multimodal information. To facilitate such reasoning, we leverage foundation models. Foundation models are particularly suited for multimodal bug detection, because they are pre-trained with code and natural language, and can be further finetuned for additional modalities. We further introduce Tiered Differential Instruction (TDI) to facilitate step-by-step reasoning that respects smart contract semantics. The key feature of \sys is that it can reason about multimodal information with verified proofs.

We extensively evaluate \sys and experiment results show that \sys generates (3.5$\times$) more accurate invariants and detects (4$\times$) more critical bugs compared to the best state-of-art tools within significantly (150$\times$) less time. Among the 270 real-world contracts verified by \sys, it has detected 32 zero-day bugs in the wild. In particular, among detected zero-day bugs, \sys has detected 5 critical zero-day vulnerabilities confirmed by developers as ``high severity.'' 

\sally{move algorithm to implementation}


\end{abstract}

\begin{comment}
 \kexin{1. Smart contracts are important but buggy and full of vulnerabilities. 
 2. One approach to detecting bugs and analyzing vulnerabilities is generate program invariants, a form of formal specification, of the smart contracts. 
 3. Existing tools rely on domain expert or developer to manually specify invariants, or dynamic analysis. Both are expensive. 
 4. We present \sys, a multi-modal foundational model, to predict invariants.
 5. Our key insight is the expected behavior (specified by invariants) of smart contract relying on understanding multimodal information....
 6. Results}


\sally{in main intro, gradually lead from transaction behavior to stateful transition}
\kexin{background. 
introduce machine un-auditable, cannot be automated, which requires understanding underlying transaction logic. 
Specifically, typical approach is to manual specify invariants - based on human reasoning/understanding of transaction logic and programing context.
Unfortunately/However, they are expensive. manual won't scale at all. 
The fundamental limitation is that existing automated analyses cannot reason across various source of information (i.e., modalities), \eg code, transaction behavior (their dynamic executions), natural language.
}
\sally{in order to reason about smart contract's different modalities... we further introduce tier of thought (ToT). Structure of Thought (SoT). change subsection name to ToT or SoT to force step by step reasoning, as well as respect smart contract semantics}
\end{comment}

==> alg/bmc.tex <==
\begin{algorithm}[!t]
\footnotesize
% \renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{2pt}
\caption{Bounded Model Checking Procedure $BMC(S, c_i, m):$}
\label{algo: bmc}
\begin{tabular}{lp{2.9in}}
\textbf{Input}:
    &an input smart contract $S$, candidate invariant $c_i$, and user-specified recursion depth $m$. \\
\textbf{Input}:
    &an SMT solver $SAT$, an initial state $s_0$, a final state $s_n$. \\
\textbf{Output}:
    & Counter Example($e$) or No Counter Examples($ne$).\\
\end{tabular}
\begin{spacing}{1.1}
\begin{algorithmic}[1]
\State $P$ $\coloneqq$ \{$S$, $c_i$, assume $s_0$, $\neg{s_n}$\};
\State  $T$ $\coloneqq$ $Open\_Call\_Sites$\{$P$\};
\For{$r$ = 0 to $m$}
  \State   stratified inline $T$ and $SAT.Assert(\forall t_i \in T)$;
  \If{$SAT.Check()$==SAT}
  \State         return $e$ = $SAT.PATH$; 
\EndIf
\State  return $ne$; 
\EndFor
\end{algorithmic}
\end{spacing}
\end{algorithm}

==> invariant_template_table.tex <==
\begin{table*}[!t]
\footnotesize
\setlength{\tabcolsep}{12pt}
\centering
\renewcommand{\arraystretch}{1.1}
\caption{\sys supported additional invariant templates. In addition to traditional smart contract invariants, \sys can generate and verify these additional types of invariants to detect functional bugs.}
\label{table:inv_lib}
\begin{tabular}{lll}
\toprule[1.1pt]
Expression & Description & Example \\ \midrule[.9pt]
\multicolumn{3}{c}{Checks whether a state variable is modified} \\ 
\texttt{Old(*)} & Returns the previous value of a state variable before it is modified again & \texttt{var == Old(var)} \\ 
\midrule[.9pt]
\multicolumn{3}{c}{Checks user-desired volatility ratio} \\ 
\texttt{Old(*) * k} & Change of key variables doesn't exceed user-specified ratio $k$ & \texttt{var $\leqslant$ Old(var) * k} \\ 
\midrule[.9pt]
\multicolumn{3}{c}{Checks cross-function and cross-contract calls} \\ 
\texttt{Modifier\{*\}} &\texttt{Modifier} specifying an entire function's behavior & \texttt{Modifier\{pre ... post\}} \\
\texttt{Invariant\{*\}} & \texttt{Invariant\{*\}} checking function return values during cross-contract calls & \texttt{Invariant\{funcA==i\}} \\
\texttt{Assume\{*\}}  & Assumed condition before a given program point  & \texttt{Assume\{var$<$i\}} \\
\texttt{Ensure\{*\}}   & Ensured condition after a given program point  & \texttt{Ensure\{var==i\}} \\
\midrule[.9pt]
\multicolumn{3}{c}{Checks comparisons between integer/bytes and mapping data types} \\ 
\texttt{SumMapping(*)} &  sum over each (key, value) pair & \texttt{bal $>$ $\sum\limits_{k=1}^k$fees[k]} \\

 \bottomrule[1.1pt]
\end{tabular}
\end{table*}

==> large_tables/ablation.tex <==
\begin{table}[!t]

\small
\setlength{\tabcolsep}{8pt}
\centering
\renewcommand{\arraystretch}{1.1}

\caption{Finetuned Model Performance. ToT-*: ToT finetuned LLaMA.
M*L: multimodal LLaMA.
S*L: single-modal LLaMA.
*OL: optimized LLaMA. 
*NL: non-optimized LLaMA. 
Alpaca: Stanford' self-instructed LLaMA.
T5: Google's T5-Small. GPT2: OpenAI's GPT2. OPT-350M: Meta's OPT-350M. }

\label{table:all_model_eval}
\rowcolors{2}{white}{gray!30}

\begin{tabular}{lllll}
\toprule
Model & Acc. & Prec. & Rec.  & F1 \\
 \midrule
% \midrule
 Alpaca \cite{Alpaca} & 0.72  & 0.72 & 0.58 & 0.65\\
% \bottomrule
% \midrule
 T5 \cite{T5} & 0.81  & 0.81 & 0.70  & 0.75\\
% \bottomrule
% \midrule
 GPT2 \cite{GPT2} & 0.57  & 0.57  & 0.20  & 0.30\\
% \bottomrule
% \midrule
OPT-350M \cite{OPT} & 0.53 & 0.53 & 0.25  & 0.34\\
LLaMA-7B \cite{LLaMA} & 0.90 & 0.90 & 0.87  & 0.88\\
\midrule
 w/o Multi \& ToT \& OPT & 0.54 & 0.54  &  0.33 & 0.41 \\
w/o ToT & 0.86 & 0.86 & 0.80 &0.83\\
w/o Multi \& ToT & 0.48  & 0.48  & 0.22 &0.30\\
 w/o Multi & 0.64 & 0.90 & 0.30 & 0.45\\

 w/o Multi. \& OPT & 0.63 & 0.90  & 0.33  & 0.45\\
 w/o OPT \cite{LLaMA} & 0.97 & 0.94 & \textbf{0.93} & 0.94\\
\midrule
Full \sys & \textbf{0.97}  &  \textbf{0.96}  & 0.92 & \textbf{0.94}\\
\bottomrule
\end{tabular}
\end{table}

==> large_tables/bug_result_table.tex <==
\begin{table*}[!h]
\centering
\caption{Bug Detection Results by Existing Tools}
\label{table:full_bug_eva}
Bug ID: CVE IDs and IDs assigned to developer confirmed bug. Loss: financial loss caused by each bug. Bug Type: MMB (multimodal bugs) and SMB (single-modal bugs). Contract: the name of each buggy contract. LOC: lines of code in a contract. Invariants: whether a tool can generate inviariants and if it does, the number of invariants generated. \#Bugs: the number of true positive bugs in a contract detected by a tool. Bug value: the total financial loss caused by the bugs that are detected by each tool. BPI: bug-preventive invariants generated by each tool. \color{red}\xmark\color{black}: a tool fails to generate invariants and/or verify a test contract with vulnerable transactional sequences. 
\color{red}error\color{black}: a tool reports internal errors on a contract. \color{green}\CheckmarkBold:\color{black}: a tool successfully generates invariants and/or verify a test contract with vulnerable transactional sequences. 
\scalebox{0.35}{
\begin{tabular}{|lllllr|lll|lll|lll|lll|lll|lll|lll|}
\hline
No.   & Bug ID       & Bug Type & Contract                   & Loss (\$m)   & \multicolumn{1}{l|}{LOC}         &            & \textbf{\sys}  &      &            & \textbf{VeriSol}  &      &            & \textbf{SmarTest} &      &            & \textbf{VeriSmart} &      &            & \textbf{Mythril}  &      &            & \textbf{Slither}  &      &            & \textbf{Manticore} &      \\
      &              &          &                            &              & \multicolumn{1}{l|}{}           & Invariants & Verified & \#Bugs & Invariants & Verified & \#Bugs & Invariants & Verified & \#Bugs & Invariants & Verified  & \#Bugs & Invariants & Verified & \#Bugs & Invariants & Verified & \#Bugs & Invariants & Verified  & \#Bugs \\ \hline
\#1   & 2023-041623   & MMB      & hundredFinance             & 11           & 222                             & 5  &  \color{green}\CheckmarkBold     & 2     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0    & \color{red}\xmark     &  \color{green}\CheckmarkBold           & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#2   & 2023-041423   & MMB      & sherlockYields             & 0.5          & 105                                 & 7  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0    & \color{red}\xmark     &  \color{green}\CheckmarkBold           & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#3   & 2023-30542   & SMB      & GovernorCompatibilityBravo & N/A          & 122                              & 4  &  \color{red}\xmark & 1     &  \color{red}\xmark       & \color{red}\xmark        &  0    & \color{red}\xmark     &  \color{red}\xmark          & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#4   & 2023-305423   & SMB      & Proxy                      & N/A          & 135                             & 6  &  \color{red}\xmark & 1     &  \color{red}\xmark       & \color{red}\xmark        &  0    & \color{red}\xmark     &  \color{red}\xmark          & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#5   & 2023-264831   & MMB      & TimelockController         & N/A          & 99                                                        & 8  &  \color{green}\CheckmarkBold & 5     &  \color{red}\xmark       & \color{red}\xmark        &  0    & \color{red}\xmark     &  \color{red}\xmark          & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#6   & 2023-26488   & SMB      & ERC721                     & 2            & 87                              & 5  &  \color{green}\CheckmarkBold & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold         &  1    & \color{red}\xmark     &  \color{green}\CheckmarkBold          & 1     & \color{green}\CheckmarkBold           &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  1    & \color{red}\xmark           & \color{red}\xmark         & 1     & \color{red}\xmark           & \color{red}\xmark          &    1 \\
\#7   & 2023-23940   & MMB      & Dao                        & 160          & 85                              & 3  &  \color{green}\CheckmarkBold & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold         &  1    & \color{red}\xmark     & \color{red}\xmark         & 0     & \color{red}\xmark          &   \color{red}\xmark           &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0 \\
\#8   & 2023-063023  & MMB      & sushiTrident               & N/A          & 231                              & 4  &  \color{red}\xmark  & 1     &  \color{red}\xmark       & \color{red}\xmark        &  0    & \color{red}\xmark     & \color{red}error         & 0     & \color{red}error          &   \color{red}\xmark           &  N/A    & \color{red}\xmark          &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0 \\

\#9   & 2023-051123  & MMB      & SellToken01                & 0.95         & 153                            & 8  &  \color{green}\CheckmarkBold     & 2     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0    & \color{red}\xmark     &  \color{green}\CheckmarkBold           & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#10  & 2023-051023  & SMB      & SNK                        & 0.19         & 81                              & 3  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  1   &   \color{red}\xmark    &  \color{green}\CheckmarkBold           & 1     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#11  & 2023-050623  & SMB      & Melo                       & 0.9          & 122                             & 2  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{red}\xmark          &  0   &   \color{red}\xmark    &  \color{red}\xmark            & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#12  & 2023-050323  & MMB      & NeverFall                  & 0.74         & 203                             & 9  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    &  \color{red}\xmark            & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#13  & 2023-050123  & MMB      & makeCall                   & 0.54         & 164                             & 6  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    &  \color{red}\xmark            & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#14  & 2023-040923  & MMB      & AUX                        & N/A          & 101                              & 3  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    &  \color{red}\xmark            & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#15  & 2023-032623  & MMB      & vote                       & 0.23         & 164                              & 9  &  \color{green}\CheckmarkBold     & 3     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    &  \color{red}\xmark            & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#16  & 2023-031323  & MMB      & EulerFinance               & 200          & 121                              & 8  &  \color{green}\CheckmarkBold     & 2     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    &  \color{red}\xmark            & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#17  & 2023-022523  & SMB      & OLIFE                      & 0.11         & 192                             & 5  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  1   &   \color{red}\xmark    &  \color{green}\CheckmarkBold            & 1     & \color{green}\CheckmarkBold           &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#18  & 2023-022023  & SMB      & Swapos                     & 0.5          & 199                             & 8  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    &  \color{red}\xmark            & 0     & \color{red}error           &   \color{red}\xmark          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#17  & 2023-022523  & SMB      & OLIFE                      & 0.11         & 192                             & 5  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  1   &   \color{red}\xmark    &  \color{green}\CheckmarkBold            & 1     & \color{green}\CheckmarkBold           &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#19  & 2023-013123  & MMB      & airToken                   & N/A          & 78                               & 7  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    &  \color{green}\CheckmarkBold            & 0     & \color{red}\xmark          &   \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#20  & 2023-012223  & SMB      & NFT                        & N/A          & 191                              & 4  &  \color{green}\CheckmarkBold     & 2     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark     &  \color{green}\CheckmarkBold            & 2     & \color{green}\CheckmarkBold          &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\

\#21  & 2023-012023  & MMB      & BEC                        & N/A          & 62                            & 3  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    &  \color{green}\CheckmarkBold            & 0     & \color{red}\xmark          &   \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\

\#22  & 2023-011123  & SMB      & Axioma                     & 0.25         & 75                              & 3  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark     &  \color{green}\CheckmarkBold            & 1     & \color{green}\CheckmarkBold          &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  1    & \color{red}\xmark           & \color{red}\xmark         & 1     & \color{red}\xmark           & \color{red}\xmark          &    1  \\
\#23  & 2022-72222   & MMB      & InverseFinance             & 7            & 201                        & 7  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    &  \color{red}error          & N/A     & \color{red}\xmark          &   \color{red}error          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\     
\#24  & 2022-310122  & MMB      & pancakeSwaplottery         & 1.8          & 208                         & 5  &  \color{green}\CheckmarkBold     & 3     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    & \color{green}\CheckmarkBold          & 0     & \color{red}\xmark         &   \color{red}error          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\     
\#25  & 2022-25806   & SMB      & moneyReserve               & 0.11         & 65    & 2  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    & \color{green}\CheckmarkBold          & 2     & \color{red}\xmark         &     \color{green}\CheckmarkBold          &  2    & \color{red}\xmark           &  \color{red}\xmark      &  1    & \color{red}\xmark           & \color{red}\xmark         & 1     & \color{red}\xmark           & \color{red}\xmark          &    1  \\     
\#26  & 2022-20234   & MMB      & pancakeswap                & 16           & 157                              & 7  &  \color{green}\CheckmarkBold     & 4     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    & \color{red}error         & N/A     & \color{red}\xmark         &   \color{red}error          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 
\#27  & 2022-20125   & MMB      & uniswap                    & 1.8          & 155                            & 6  &  \color{green}\CheckmarkBold     & 2     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    & \color{red}error         & N/A     & \color{red}\xmark         &   \color{red}error          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}{\xmark}          &    0  \\ 
\#28  & 2022-20007   & MMB      & visor                      & 8            & 72                             & 3  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{green}\CheckmarkBold         &   \color{green}\CheckmarkBold          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 
\#29  & 2022-110222  & MMB      & DFX                        & 5            & 121    & 5  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{green}\CheckmarkBold         &   \color{green}\CheckmarkBold          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 
\#30  & 2022-100922  & MMB      & LIFI                       & 600          & 267                             & 5  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}error    & \color{red}error        & N/A     & \color{red}error        &  \color{red}error          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 

\#31  & 2022-092222  & SMB      & moon                       & 0.1          & 152                             & 3  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    &  \color{green}\CheckmarkBold            & 1     & \color{green}\CheckmarkBold          &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 1     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#32  & 2022-0910122 & SMB      & VASPIndex                  & N/A          & 98   & 2  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark     &  \color{green}\CheckmarkBold            & 1     & \color{green}\CheckmarkBold          &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 1     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#33  & 2022-083122  & SMB      & proxyTransfer              & N/A          & 211                            & 5  &  \color{green}\CheckmarkBold     & 2     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark     &  \color{green}\CheckmarkBold            & 2     & \color{green}\CheckmarkBold          &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0 & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#34  & 2022-080222  & MMB      & Nomad                      & 190          & 231            & 6  &  \color{green}\CheckmarkBold     & 3     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}error    & \color{red}error        & N/A     & \color{red}error        &  \color{red}error          &  N/A    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 

\#35  & 2022-062422  & MMB      & Fundstransfer              & 0.12         & 191                            & 3  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    & \color{green}\CheckmarkBold        & 0     & \color{green}\CheckmarkBold    & \color{green}\CheckmarkBold          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 

\#36  & 2022-053222  & MMB      & walnutFinance              & 0.5          & 208                          & 6  &  \color{green}\CheckmarkBold     & 2     &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 

\#37  & 2022-051022  & SMB      & LFW                        & N/A          & 78                             & 2  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark     &  \color{green}\CheckmarkBold            & 1     & \color{green}\CheckmarkBold          &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  1    & \color{red}\xmark           & \color{red}\xmark         & 1     & \color{red}\xmark           & \color{red}\xmark          &    1  \\    
\#38  & 2022-050822  & MMB      & Fortress Loan             & 5 &98  &  9  &  \color{green}\CheckmarkBold    & 3    &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 

\#39  & 2022-050222  & MMB      & Meter                      & 4.4          & 159                             & 6  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 

\#40  & 2022-040922  & MMB      & FeiProtocol                & 80           & 133                           & 6  &  \color{green}\CheckmarkBold     & 2     &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 
\#41  & 2022-030722  & MMB      & revest                     & 11.2         & 201                             & 5  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 
\#42  & 2022-030422  & MMB      & Cartel                     & 0.56         & 59                              & 2  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 
\#43  & 2022-012822  & MMB      & Qubit                      & 80           & 212                            & 7  &  \color{green}\CheckmarkBold     & 3     &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 

\#44  & 2022-012022  & MMB      & KYC                        & 0.33         & 195                            & 5  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 

\#45  & 2021-52021   & MMB      & PancakeBunny               & 200          & 199                           & 5  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 

\#46  & 2021-3006    & MMB      & seal                       & 0.32         & 208                           & 5  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 
\#47  & 2021-123122  & SMB      & DSProxyCache               & N/A          & 101                             & 9  &  \color{green}\CheckmarkBold     & 3     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  1   &   \color{red}\xmark     &  \color{green}\CheckmarkBold            & 1     & \color{green}\CheckmarkBold          &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  1    & \color{red}\xmark           & \color{red}\xmark         & 1     & \color{red}\xmark           & \color{red}\xmark          &    0  \\    
\#48  & 2021-123121  & MMB      & bunnyswap                  & 2            & 207                              & 5  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 
\#49  & 2021-120221  & MMB      & MonoX                      & 30           & 153                           & 7  &  \color{green}\CheckmarkBold     & 3     &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 
\#50  & 2021-102721  & MMB      & CreamFinance               & 130          & 222                            & 7  &  \color{green}\CheckmarkBold     & 2    &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 

\#51  & 2021-102321  & SMB      & payout                     & 0.2          & 55                             & 3  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark     &  \color{green}\CheckmarkBold            & 1     & \color{green}\CheckmarkBold          &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  1    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\    
\#52  & 2021-091721  & MMB      & sushiSwap                  & 3            & 122                              & 5  &  \color{green}\CheckmarkBold     & 3    &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 
\#53  & 2021-081121  & MMB      & polynetwork                & 610          & 220                             & 7  &  \color{green}\CheckmarkBold     & 1    &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\

\#54  & 2021-071021  & MMB      & ChainSwap                  & 8            & 199              & 5  &  \color{green}\CheckmarkBold     & 2    &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ 

\#55  & 2021-052221  & SMB      & TAO                        & N/A          & 79     & 2  &  \color{green}\CheckmarkBold     & 1     &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  1   &   \color{red}\xmark     &  \color{green}\CheckmarkBold            & 1     & \color{green}\CheckmarkBold          &   \color{green}\CheckmarkBold           &  1    & \color{red}\xmark           &  \color{red}\xmark      &  1    & \color{red}\xmark           & \color{red}\xmark         &  1    & \color{red}\xmark           & \color{red}\xmark          &    1 \\    
\#56  & 2021-050321  & MMB      & tokenMarket                & 1            & 199      & 3  &  \color{green}\CheckmarkBold     & 1    &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#57  & 2020-35962   & MMB      & LRC                        & 0.11         & 210   & 3  &  \color{green}\CheckmarkBold     & 1    &  \color{red}\xmark       & \color{red}\xmark           &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#58  & 2020-17753   & SMB      & tokensale                  & 0.04         & 207 & 3  &  \color{green}\CheckmarkBold     & 1    &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#59  & 2019-19831   & SMB      & BOMBBA                     & 0.2          & 216                           & 4  &  \color{green}\CheckmarkBold     & 1    &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\
\#60  & 2018-19830   & SMB      & BAFCToken                  & 0.15         & 220                             & 3  &  \color{green}\CheckmarkBold     & 1    &  \color{red}\xmark       & \color{green}\CheckmarkBold          &  0   &   \color{red}\xmark    & \color{red}\xmark         & 0     & \color{red}\xmark    & \color{red}\xmark          &  0    & \color{red}\xmark           &  \color{red}\xmark      &  0    & \color{red}\xmark           & \color{red}\xmark         & 0     & \color{red}\xmark           & \color{red}\xmark          &    0  \\ \hline
      &              &          &                           &              & \multicolumn{1}{l|}{}           &            &     \#Bugs:      &  94    &            &     \#Bugs:     &   7   &            &     \#Bugs:      &   15   &            &  \#Bugs:   & 14     &            &   \#Bugs:    & 7     &            &   \#Bugs:   &   8   &            &   \#Bugs: &  5    \\
\textbf{Total} &              &          & \textbf{60 contracts}               & \textbf{\$2372.85(m)} & \multicolumn{1}{l|}{\textbf{9281 lines}} &            &      bug value:   & \$2372.85m       &             &      bug value:   & \$165.41m       &            &        bug value:  &  \$366.75m    &            &        bug value:    & \$2.67m      &            &      bug value:    &  \$9.20m     &            &   bug value:        &  \$9.21m     &            &    bug value:        &  \$2.35m     \\
      &              &          &                            &              & \multicolumn{1}{l|}{}           &            &   BPI:       & 100\%     &            &    BPI:     &  11.67\%       &            &  BPI:         &  0\%    &            &     Bug-Preventive Invariants:        &   14\%   &            &    BPI:      &   0\%     &            &  BPI:   &  0\%     &            &     BPI:      &  0\%     \\ \hline

\end{tabular}}
\end{table*}


==> large_tables/invariant_result_table.tex <==
\begin{table*}[!h]
\centering
\caption{Invariants Detection Results by Existing Tools}
\label{table:original_inv_table}
Benchmark: 30 contracts from InvCon's own benchmark and 30 contracts from VeriSol's own benchmark. LOC: lines of code. Output Invariants: a tool can output inferred invariants directly; verified: a tool can verify inferred invariants. \#FP: the number of false positive invariants generated by a tool. Validity Ratio: if a tool can generate invariants with $\leqslant$ 1 false positive invariant, then it's considered a valid result.
\color{red}\xmark\color{black}: a tool cannot output invariants or verify inferred invariants.
\color{red}error\color{black}: a tool fail to detect or verify invariants on a test contract.  \color{green}\CheckmarkBold:\color{black}: a tool successfully generates invariants and/or verify a test contract.
\scalebox{0.55}{
\begin{tabular}{|llr|llr|lll|lll|}
\hline
Benchmark      & No.                   & \multicolumn{1}{l|}{LOC} &                             & \textbf{\sys}               & \multicolumn{1}{l|}{}                                                           &                             & \textbf{InvCon}         &                                   &                      & \textbf{VeriSol}            &              \\
               &                       & \multicolumn{1}{l|}{}    & Output Invariants           & Verified                    & \multicolumn{1}{l|}{\#FP}                                                       & Output Invariants           & Verified                & \#FP                              & Output Invariants    & Verified                    & \#FP         \\ \hline
               & \#1                    & 102                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{5}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#2                    & 99                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{9}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#3                    & 201                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{4}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#4                    & 98                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{3}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#5                    & 111                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{5}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#6                    & 152                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 2                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{2}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#7                    & 213                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{1}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#8                    & 139                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{4}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#9                    & 129                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{2}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#10                   & 199                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 1                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{1}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#11                   & 201                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{5}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#12                   & 244                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 1                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{4}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#13                   & 231                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{2}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#14                   & 211                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{2}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
InvCon         & \#15                   & 100                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{3}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#16                   & 101                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 1                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{4}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#17                   & 231                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{1}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#18                   & 201                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{9}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#19                   & 50                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{9}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#20                   & 95                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{8}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#21                   & 54                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{7}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#22      & 231                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{9}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#23                   & 111                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{2}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#24                   & 154                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{5}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#25                   & 177                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{1}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#26                   & 167                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{4}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#27                   & 172                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{9}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#28                   & 122                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{10}           & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#29                   & 99                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{3}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#30                   & 81                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{green}\CheckmarkBold & \color{red}\xmark       & \multicolumn{1}{r|}{2}            & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\\hline
               &\#1                    & 45                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#2                    & 16                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#3                    & 28                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#4                    & 55                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#5                    & 31                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#6                    & 29                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#7                    & 61                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#8                    & 101                      & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#9                    & 32                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#10                   & 22                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#11                   & 18                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#12                   & 10                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#13                   & 5                        & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#14                   & 34                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
VeriSol        & \#15                   & 19                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#16                   & 22                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#17                   & 23                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#18                   & 21                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#19                   & 15                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#20                   & 19                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#21                   & 17                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#22                   & 59                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 1                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#23                   & 32                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#24                   & 15                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#25                   & 21                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#26                   & 20                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#27                   & 19                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#28                   & 34                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#29                   & 15                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\
               & \#30                   & 40                       & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold & 0                                                                               & \color{red}\xmark           & \color{red}\xmark       & \color{red}error                  & \color{red}\xmark    & \color{green}\CheckmarkBold & N/A          \\ \hline
               &                       &     &                             & \textbf{Validity Ratio}     & \textbf{98.3\%} &                             & \textbf{Validity Ratio} & \textbf{6.67\%}                   &                      & \textbf{Validity Ratio}     & \textbf{N/A} \\
\textbf{Total} & \textbf{60 contracts} & \textbf{5354}            & \textbf{60 contracts}       & \textbf{60 contracts}       & \textbf{6}                                                                      & \textbf{30 contracts}       & \textbf{30 contracts}   & {\textbf{135}} & \textbf{0 contracts} & \textbf{60}                 & \textbf{N/A} \\ \hline
\end{tabular}}
\end{table*}



==> large_tables/listing2_solution.tex <==
\begin{table}[!t]
\footnotesize
\setlength{\tabcolsep}{4pt}
\centering
\renewcommand{\arraystretch}{1.1}
\caption{\sys inferred invariants in Listing 2.}
\label{table:short_motivating_invariants}
\begin{tabular}{ll}
\toprule[1.1pt]
Critical Program Points & Inferred Invariants \\ \midrule[.9pt]
{17+}  & \texttt{assert(price <= Old(price)*k);}   \\
 \bottomrule[1.1pt]
\end{tabular}\\

\scriptsize
17+ refers to the line-numbered location where the invariant should be inserted, \eg 17+ means immediately after line 17. \texttt{Old()} is a widely used invariant instrumentation to obtain a variable value during previous program execution state before a function is invoked.  \texttt{Old(price)} returns the price point before \texttt{liquidate} function is called. k is an adjustable ratio, where \sys sets default as k=2.
\end{table}

==> large_tables/modality_table.tex <==
\begin{table}[!t]
\small
\setlength{\tabcolsep}{10pt}
\centering
\renewcommand{\arraystretch}{1.1}

\caption{Existing tools' modality analysis. SC: source code. NL: natural language.}
\label{table:tool_modality}
\begin{tabular}{l|llll}
\toprule
\multirow{2}{*}{\bf Tools} &   \multicolumn{2}{c}{\bf Multimodalities}  \\
               & SC  & NL       \\ \midrule
\sys           & \color{green}\CheckmarkBold & \color{green}\CheckmarkBold  \\
\verisol        & \color{green}\CheckmarkBold & \color{red}\xmark                        \\
\invcon         & \color{green}\CheckmarkBold & \color{red}\xmark                 \\
\smartest      & \color{green}\CheckmarkBold & \color{red}\xmark                  \\
\verismart      & \color{green}\CheckmarkBold & \color{red}\xmark                 \\
\mythril        & \color{green}\CheckmarkBold & \color{red}\xmark                \\
\slither        & \color{green}\CheckmarkBold & \color{red}\xmark                         \\
\manticore      & \color{green}\CheckmarkBold & \color{red}\xmark                \\ \bottomrule
\end{tabular}
\end{table}

==> large_tables/sys_bug_result.tex <==
\begin{table*}[!h]
\centering
\caption{\sys Bug Detection Result Breakdown
}
\label{table:bug_result_breakdown}
Bug ID: CVE IDs and IDs assigned to developer confirmed bug. Loss: financial loss caused by each bug. Bug Type: MMB (multimodal bugs) and SMB (single-modal bugs). Contract: the name of each buggy contract. LOC: lines of code in a contract. Invariants: whether a tool can generate inviariants and if it does, the number of invariants generated. \#Bugs: the number of true positive bugs in a contract detected by a tool. Bug value: the total financial loss caused by the bugs that are detected by each tool. BPI: bug-preventive invariants generated by each tool. \color{red}\xmark\color{black}: a tool fails to generate invariants and/or verify a test contract with vulnerable transactional sequences. 
\color{red}error\color{black}: a tool reports internal errors on a contract. \color{green}\CheckmarkBold:\color{black}: a tool successfully generates invariants and/or verify a test contract with vulnerable transactional sequences. 
\begin{tabular}{|llllr|lll|}
\hline
No.            & Bug ID       & Bug Type & Contract                   & \multicolumn{1}{l|}{LOC}        &            & \textbf{\sys}               &            \\
               &              &          &                            & \multicolumn{1}{l|}{}           & Invariants & Verified                    & \#Bugs     \\ \hline
\#1            & 2023-041623  & MMB      & hundredFinance             & 222                             & 5          & \color{green}\CheckmarkBold & 2          \\
\#2            & 2023-041423  & MMB      & sherlockYields             & 105                             & 7          & \color{green}\CheckmarkBold & 1          \\
\#3            & 2023-30542   & SMB      & GovernorCompatibilityBravo & 122                             & 4          & \color{red}\xmark           & 1          \\
\#4            & 2023-305423  & SMB      & Proxy                      & 135                             & 6          & \color{red}\xmark           & 1          \\
\#5            & 2023-264831  & MMB      & TimelockController         & 99                              & 8          & \color{green}\CheckmarkBold & 5          \\
\#6            & 2023-26488   & SMB      & ERC721                     & 87                              & 5          & \color{green}\CheckmarkBold & 1          \\
\#7            & 2023-23940   & MMB      & Dao                        & 85                              & 3          & \color{green}\CheckmarkBold & 1          \\
\#8            & 2023-063023  & MMB      & sushiTrident               & 231                             & 4          & \color{red}\xmark           & 1          \\
\#9            & 2023-051123  & MMB      & SellToken01                & 153                             & 8          & \color{green}\CheckmarkBold & 2          \\
\#10           & 2023-051023  & SMB      & SNK                        & 81                              & 3          & \color{green}\CheckmarkBold & 1          \\
\#11           & 2023-050623  & SMB      & Melo                       & 122                             & 2          & \color{green}\CheckmarkBold & 1          \\
\#12           & 2023-050323  & MMB      & NeverFall                  & 203                             & 9          & \color{green}\CheckmarkBold & 1          \\
\#13           & 2023-050123  & MMB      & makeCall                   & 164                             & 6          & \color{green}\CheckmarkBold & 1          \\
\#14           & 2023-040923  & MMB      & AUX                        & 101                             & 3          & \color{green}\CheckmarkBold & 1          \\
\#15           & 2023-032623  & MMB      & vote                       & 164                             & 9          & \color{green}\CheckmarkBold & 3          \\
\#16           & 2023-031323  & MMB      & EulerFinance               & 121                             & 8          & \color{green}\CheckmarkBold & 2          \\
\#17           & 2023-022523  & SMB      & OLIFE                      & 192                             & 5          & \color{green}\CheckmarkBold & 1          \\
\#18           & 2023-022023  & SMB      & Swapos                     & 199                             & 8          & \color{green}\CheckmarkBold & 1          \\
\#17           & 2023-022523  & SMB      & OLIFE                      & 192                             & 5          & \color{green}\CheckmarkBold & 1          \\
\#19           & 2023-013123  & MMB      & airToken                   & 78                              & 7          & \color{green}\CheckmarkBold & 1          \\
\#20           & 2023-012223  & SMB      & NFT                        & 191                             & 4          & \color{green}\CheckmarkBold & 2          \\
\#21           & 2023-012023  & MMB      & BEC                        & 62                              & 3          & \color{green}\CheckmarkBold & 1          \\
\#22           & 2023-011123  & SMB      & Axioma                     & 75                              & 3          & \color{green}\CheckmarkBold & 1          \\
\#23           & 2022-72222   & MMB      & InverseFinance             & 201                             & 7          & \color{green}\CheckmarkBold & 1          \\
\#24           & 2022-310122  & MMB      & pancakeSwaplottery         & 208                             & 5          & \color{green}\CheckmarkBold & 3          \\
\#25           & 2022-25806   & SMB      & moneyReserve               & 65                              & 2          & \color{green}\CheckmarkBold & 1          \\
\#26           & 2022-20234   & MMB      & pancakeswap                & 157                             & 7          & \color{green}\CheckmarkBold & 4          \\
\#27           & 2022-20125   & MMB      & uniswap                    & 155                             & 6          & \color{green}\CheckmarkBold & 2          \\
\#28           & 2022-20007   & MMB      & visor                      & 72                              & 3          & \color{green}\CheckmarkBold & 1          \\
\#29           & 2022-110222  & MMB      & DFX                        & 121                             & 5          & \color{green}\CheckmarkBold & 1          \\
\#30           & 2022-100922  & MMB      & LIFI                       & 267                             & 5          & \color{green}\CheckmarkBold & 1          \\
\#31           & 2022-092222  & SMB      & moon                       & 152                             & 3          & \color{green}\CheckmarkBold & 1          \\
\#32           & 2022-0910122 & SMB      & VASPIndex                  & 98                              & 2          & \color{green}\CheckmarkBold & 1          \\
\#33           & 2022-083122  & SMB      & proxyTransfer              & 211                             & 5          & \color{green}\CheckmarkBold & 2          \\
\#34           & 2022-080222  & MMB      & Nomad                      & 231                             & 6          & \color{green}\CheckmarkBold & 3          \\
\#35           & 2022-062422  & MMB      & Fundstransfer              & 191                             & 3          & \color{green}\CheckmarkBold & 1          \\
\#36           & 2022-053222  & MMB      & walnutFinance              & 208                             & 6          & \color{green}\CheckmarkBold & 2          \\
\#37           & 2022-051022  & SMB      & LFW                        & 78                              & 2          & \color{green}\CheckmarkBold & 1          \\
\#38           & 2022-050822  & MMB      & Fortress Loan              & 98                              & 9          & \color{green}\CheckmarkBold & 3          \\
\#39           & 2022-050222  & MMB      & Meter                      & 159                             & 6          & \color{green}\CheckmarkBold & 1          \\
\#40           & 2022-040922  & MMB      & FeiProtocol                & 133                             & 6          & \color{green}\CheckmarkBold & 2          \\
\#41           & 2022-030722  & MMB      & revest                     & 201                             & 5          & \color{green}\CheckmarkBold & 1          \\
\#42           & 2022-030422  & MMB      & Cartel                     & 59                              & 2          & \color{green}\CheckmarkBold & 1          \\
\#43           & 2022-012822  & MMB      & Qubit                      & 212                             & 7          & \color{green}\CheckmarkBold & 3          \\
\#44           & 2022-012022  & MMB      & KYC                        & 195                             & 5          & \color{green}\CheckmarkBold & 1          \\
\#45           & 2021-52021   & MMB      & PancakeBunny               & 199                             & 5          & \color{green}\CheckmarkBold & 1          \\
\#46           & 2021-3006    & MMB      & seal                       & 208                             & 5          & \color{green}\CheckmarkBold & 1          \\
\#47           & 2021-123122  & SMB      & DSProxyCache               & 101                             & 9          & \color{green}\CheckmarkBold & 3          \\
\#48           & 2021-123121  & MMB      & bunnyswap                  & 207                             & 5          & \color{green}\CheckmarkBold & 1          \\
\#49           & 2021-120221  & MMB      & MonoX                      & 153                             & 7          & \color{green}\CheckmarkBold & 3          \\
\#50           & 2021-102721  & MMB      & CreamFinance               & 222                             & 7          & \color{green}\CheckmarkBold & 2          \\
\#51           & 2021-102321  & SMB      & payout                     & 55                              & 3          & \color{green}\CheckmarkBold & 1          \\
\#52           & 2021-091721  & MMB      & sushiSwap                  & 122                             & 5          & \color{green}\CheckmarkBold & 3          \\
\#53           & 2021-081121  & MMB      & polynetwork                & 220                             & 7          & \color{green}\CheckmarkBold & 1          \\
\#54           & 2021-071021  & MMB      & ChainSwap                  & 199                             & 5          & \color{green}\CheckmarkBold & 2          \\
\#55           & 2021-052221  & SMB      & TAO                        & 79                              & 2          & \color{green}\CheckmarkBold & 1          \\
\#56           & 2021-050321  & MMB      & tokenMarket                & 199                             & 3          & \color{green}\CheckmarkBold & 1          \\
\#57           & 2020-35962   & MMB      & LRC                        & 210                             & 3          & \color{green}\CheckmarkBold & 1          \\
\#58           & 2020-17753   & SMB      & tokensale                  & 207                             & 3          & \color{green}\CheckmarkBold & 1          \\
\#59           & 2019-19831   & SMB      & BOMBBA                     & 216                             & 4          & \color{green}\CheckmarkBold & 1          \\
\#60           & 2018-19830   & SMB      & BAFCToken                  & 220                             & 3          & \color{green}\CheckmarkBold & 1          \\ \hline
               &              &          &                            & \multicolumn{1}{l|}{}           &            & \#Bugs:                     & 94         \\
\textbf{Total} &              &          & \textbf{60 contracts}      & \multicolumn{1}{l|}{9281 lines} &            & bug value:                  & \$2372.85m \\
               &              &          &                            & \multicolumn{1}{l|}{}           &            & BPI:                        & 100\%      \\ \hline
\end{tabular}
\end{table*}

==> motivation.tex <==

\begin{lstlisting}
1 contract TimelockController {
2     struct Proposal {
3         uint160 sTime; address newOwner;
4         }
5         IERC20 votingToken;
6         address owner;
7         Proposal proposal;

8      function startExecute() external {
9         require(proposal.sTime == 0, 
                  "on-going proposal");
10         proposal = Proposal(block.timestamp, 
                               msg.sender);
11     }
12     function execute(uint amount) external {
13         require(proposal.sTime + 24 hours > block.timestamp,
14               "execution has ended");
15         votingToken.transferFrom(
16              msg.sender, address(this), amount);       
       //Old(votingToken) = votingToken; 
       //pre condition invariant #1: 
       //Precondition(Old(votingToken) == votingToken);
17     }
18     function endExecute() external {
19        require(proposal.sTime != 0, "no proposal");
20         require(proposal.sTime + 24 hours < block.timestamp,
21           "execution has not ended");
        //post condition invariant #2:   
        //Postcondition(Old(votingToken) == votingToken); 
22        require(
            votingToken.balanceOf(address(this))*2
23            > votingToken.totalSupply(),            
              "execution failed");
24            owner = findHighest(_allProposals);
25            delete proposal;
26    }
31     function getFunds() external onlyOwner {
            //adversarial condition holds after verification
           //contextual warning: pause()
32         return allLockedTokens; 
33     }
34 }
\end{lstlisting}
\hspace*{1cm}EXAMPLE 1. Redacted OpenZeppelin Exploit
We provide a real-world contract to illustrate why finetuned multimodal foundation models are particularly suitable for inferring invariants against challenging bugs. Example 1 is a multimodal privilege escalation (PE) bug that existing tools fail to detect correctly. To show the effectiveness of our methodology, we also compare the outputs from optimized LLaMA finetuned on single modality v.s. on multi modality in figure 1, as well as the outputs without CoT v.s. with CoT in figure 2. 

Example 1 shows a redacted privilege escalation vulnerability of OpenZepplin's TimeController contract identified by an anonymous white hat hacker  \cite{4, 36}. This contract allows a user to start a proposal and to transfer tokens per proposal. After each 24-hour proposal round ends, the proposal that has the highest bidding becomes the new owner and will get all locked tokens. Lines 2-7 initialize 1 global struct and 3 state variables. The \texttt{Proposal\{\}} struct includes a starting time \texttt{sTime} and a new owner who initializes the proposal \texttt{newOwner}. Lines 5-7 are state variables.  \texttt{votingToken} uses IERC20 wraparound library contract and tracks how many tokens a user would like to vote when calling the \texttt{execute()} function. Note that the  IERC20 wraparound library contract has its own \texttt{transferForm()} function. Therefore, any variable declared with IERC20 can invoke \texttt{transferForm()} directly. \texttt{owner} denotes a proposal's owner. Lines 8-11 are the \texttt{startExecute()} function that sets a proposal's starting time. In particular, line 9 ensures each proposal is atomic when it's been executed. Lines 12-17 execute a proposal by first performing a check that the proposal round hasn't expired and secondly transferring the voting tokens. Lines 18-26  are the \texttt{endExecute()} function that ends a proposal round and selects the new owner. In particular, it performs three checks before a new owner is selected. First, it checks whether there is still an on-going proposal at line 19; second, it checks that the proposal round hasn't surpassed 24 hours at lines 20-21. third, it checks that more than 50\% of proposal owners in the pool have voted. When all checks are passed, line 24-25 selects a new contract owner with highest bidding and then delete the proposal round. Lines 31-34 is a privileged \texttt{getFunds()} function that allows the new contract owner from line 24 to get all locked tokens. On the surface, the logic of the contract seems sound: note that line 13 and line 19 strictly restrict \texttt{execute()} and \texttt{endExecute()} functions invocation time, where an on-going proposal cannot invoke both functions at the same time. As the contract developer(s) intended, \texttt{execute()} and \texttt{endExecute()} cannot be invoked within a single transaction in order to prevent flash loan attacks.

 However, the key vulnerability lies in the contract developer(s)' assumption that each of the three functions -\texttt{startExecute()}, \texttt{Execute()}, \texttt{endExecute()} - would be invoked sequentially in a proposal round. A white hacker launched a privilege escalation hack via bypassing the \texttt{Execute()} function and invoking the privileged \texttt{getFunds()} function directly. The hacker borrowed a large flash loan using an AMM contract and injected the flash loan as \texttt{votingToken}. Then the hacker invoked \texttt{transferForm()} in the IERC20 library contract directly without going through \texttt{execute()} function. Afterwards, the hacker ended the proposal round by invoking \texttt{endExecute()} function and became the new owner of the contract at line 24. This exploit allowed the hacker to invoke the highly privileged \texttt{getFunds()} function to obtain all locked tokens and to pay back flash loan with a profit. Detecting such privilege escalation bug is particularly challenging, because it require understanding of inter-contract communications, its business contexts, and its programming functionalities.
\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=Java,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\small\ttfamily},
  numbers=none,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=false,
  breakatwhitespace=true,
  tabsize=3
}

\begin{comment}
\begin{lstlisting}
1 pragma solidity ^0.4.24;
2 contract testLoops {
     
3     uint x = n; uint y = 0;
4     constructor(uint n) public {
5         require (n >= 0);
6         uint y = 0;
7         for (uint x = n; x != 0; x --) {
8             y++;
9         }
10     }
    //invariant #1: assert(x+y==n); 
11    function loopOne(uint n) public {
12         require (n >= 0);
    //invariant #2: assert(y==n); 
13         uint y = 0;
14         uint x = n;
15         while (x != 0) {
16             y++;
17             x--;
18        }
    //invariant #3: assert(x+y==n); 
19     } 

20     function loopTwo(uint n) public {
21         uint y = 0;
22         uint x = n;
23         do {
24             y++;
25             x--;
26         } while (x != 0);
    //invariant #4: assert(y==n); 
27     }
   //invariant #5: assert(x+y==n); 
28 }
\end{lstlisting}
\hspace*{1cm}EXAMPLE 2. Contract with Loops

To detect the bug in example 1, Guanaco uses finetuned LLaMA to identify a warning invariant in the form of a \texttt{pause()} command at the the critical line 32. Our backbone model is able to detect the accurate warning invariant, because it has learned similar contexts and semantics during finetuning. Therefore, when we test the model with a new, different buggy contract, the model can transfer its previous learning to new contexts and reason about invariants during inference.


 Example 2 is a simple contract containing three variables - $x$, $y$, $n$ - and three loops from Azure Blockchain  \cite{40}. One for loop is in the constructor and two while loops are in the \texttt{loopOne()} and \texttt{loopTwo()} functions. Upon manual checking, this contract is both programming-wise and context-wise correct. Proving correctness requires reasoning about loop and algebraic invariants in abstract sense. Automated reasoning about loop invariants has been an on-going challenge that programming language researchers actively grapple with  \cite{37, 38, 39}.

To prove correctness of example 2, Guanaco first identifies critical correct program points at lines 10, 12, 18, 26, and 27, and then generates accurate loop invariants at identified program points. After completing invariant inference, Guanaco feeds the inferred invariants into our verifier to derive proof (\textsection3.4).\\
\hspace*{0.5cm}\textbf{\textit{Gap in Existing Solutions.}} When we run existing tools [10-19] on example 1, they cannot discover or be adapted to discover the privilege escalation bug, because this contract is programming-wise sound on the surface. Existing invariants detectors and verifiers such as InvCon and VeriSol cannot be easily adapted to solve this problem, because they rely on checking arithmetic safety property. But the privilege escalation bug in this case is arithmetically sound. This bug can be detected only if one understands the intended purposes of this contract. Annotating smart contract invariants in the traditional sense, i.e. assertions and require statements, demands developers' foresight of privilege escalation. In reality, such foresight is frequently lost when a contract has complex inter-contract communications. To effectively detecting contextual bugs, a tool should possess both contextual knowledge and programming analytical ability. \\
\hspace*{0.5cm} On example 2, we observe that highly precise invariants such as line-numbered assertions are very useful for proving program correctness. However, existing smart contract verifiers  \cite{18, 20, 21} require manual sepcification of invariants, which is a both laborious and error-prone process. Existing smart contract invariant detectors  \cite{22, 23} generate invariants by extracting already-deployed contracts on blockchain and output invariants without any program points. The lack of precise program points makes inferred invariants from existing solutions much less useful. Since deployed contracts are immutable and open on the web, detecting post-deployment invariants defeats the purpose of finding bugs before hacks occur. Furthermore, existing invariants detectors are not ideal, because they also contain high false positives due to imprecise mappings between solidity and Java usesd by Daikon. \\

\end{comment}

As figure 1 shows, when a foundation model (LLaMA in this case) is finetuned on single modality, the model repeats the existing single modal invariants. In our motivating example, single modal Guananco can only infer the single modal invariant - a solidity built-in require statement - at line 19. By comparison, multi-modal Guanaco can infer an invariant condition that the value of \texttt{votingToken} should stay the same within a proposal round between lines 16 -26. 

\begin{figure*}[h]
\caption{Chain of Thought}
\includegraphics[width=1.0\textwidth]{heatmap.jpg}
\label{fig}
\end{figure*}

Guanaco first infers the bug-prone state variable \texttt{votingToken} at line 16 by tracking its key state transitions: \texttt{Old(votingToken)} = \texttt{votingToken}. Using our tailored invariant template library, Guanco infers a precondition after line 16: \texttt{Precondition(Old(votingToken)}==
\texttt{votingToken)}. After pre-condition inference, Guanaco infers the post condition after line 21: Postcondition(\texttt{Old(votingToken)} == \texttt{votingToken}). If a malicious actor bypasses the \texttt{execute()} function and injects a large flashloan in  \texttt{endExecute()} function directly, then \texttt{votingToken} variable  would transition to a wrong state (\texttt{Old(votingToken)} != \texttt{votingToken}). Our verifier would detect adversarial cases in the event that wrong transition happens. Since Guanaco formally verifies the inferred invariants and detects adversarial cases, at last it infers a \texttt{pause()} command after line 31. The predicted \texttt{pause()} command indicates the program point where transactions should be paused due to verified occurrence of adversarial conditions. 

By comparison, state-of-art tools such as Slither, Manticore, VeriSmart, and VeriSol (without Guanaco's library and specified invariants) consider this contract as safe. This bug is very challenging for existing tools, because catching it requires understanding of inter-contract communications and developers' intended atomicity of function calls. Existing tools do not possess the ability to reason about smart contracts' business contexts or developers intentions. They also frequently miss inter-contract communications. However, Guanaco can detect this challenging bug by transfer similar contexts learned from training data set and invariant templates.  



\begin{figure}
\caption{Single Modality v.s. Multi-Modality}
\includegraphics[width=0.5\textwidth]{single-multi.jpg}
\end{figure}

Figure 2 demonstrates that CoT finetuning helps Guanaco to contextualize critical programming points and contract behavior intended by developers. We compare the detection results on example 1 without CoT and with CoT. Without CoT finetuning, Guanaco miss the inference steps of invariants generation and jumps to the \texttt{pause()} command directly. The lack of inference steps in example 2 would miss the detection of adversarial cases and lead to failed verification. By comparison, CoT finetuned Gunanco can reason incrementally from program points to multimodal invariants, and then to the \texttt{pause()} command at the last problematic line. This result shows that CoT is necessary for effective multimodal invariants inference and verification. 

